F8Net: Fixed-Point 8-bit Only Multiplication for Network Quantization

Neural network quantization is a promising compression technique to reduce memory footprint and save energy consumption, potentially leading to real-time inference. However, there is a performance gap between quantized and full-precision models. To reduce it, existing quantization approaches require high-precision INT32 or full-precision multiplication during inference for scaling or dequantization. This introduces a noticeable cost in terms of memory, speed, and required energy. To tackle these issues, we present F8Net, a novel quantization framework consisting of only fixed-point 8-bit multiplication. To derive our method, we first discuss the advantages of fixed-point multiplication with different formats of fixed-point numbers and study the statistical behavior of the associated fixed-point numbers. Second, based on the statistical and algorithmic analysis, we apply different fixed-point formats for weights and activations of different layers. We introduce a novel algorithm to automatically determine the right format for each layer during training. Third, we analyze a previous quantization algorithm -- parameterized clipping activation (PACT) -- and reformulate it using fixed-point arithmetic. Finally, we unify the recently proposed method for quantization fine-tuning and our fixed-point approach to show the potential of our method. We verify F8Net on ImageNet for MobileNet V1/V2 and ResNet18/50. Our approach achieves comparable and better performance, when compared not only to existing quantization techniques with INT32 multiplication or floating-point arithmetic, but also to the full-precision counterparts, achieving state-of-the-art performance.

==> figs/fig_fix_point_mult_std_of_model.tex <==
\begin{figure}[h]
\centering
\begin{minipage}[t] {.49\linewidth}
\begin{center}
\includegraphics[width=.95\linewidth]{imgs/fix_point_multiplication.pdf}
\setlength{\tabcolsep}{0\linewidth}
\caption{An example of 8-bit fixed-point multiplication, where the two inputs are of the formats (8, 3) and (8, 4), namely 3- and 4-bit for the fractional part. The product is quantized as (8, 3) where quantization error is introduced accordingly.}\label{fig:sameC_diffM}
\end{center}
\end{minipage}\hfill
\begin{minipage}[t] {.49\linewidth}
\begin{center}
\includegraphics[width=.95\linewidth]{imgs/std_fix_quant_error_analysis_8bit_signed_False.pdf}
\setlength{\tabcolsep}{0\linewidth}
\caption{The first and second row (also the third and fourth row) share the same motion code but with different content codes.}\label{fig:sameM_diffC}
\end{center}
\end{minipage}
\end{figure}

==> figs/fig_format_vs_layer.tex <==
% \begin{figure*}[t]
% \centering
% % \vspace*{-8ex}
% % \hspace*{1ex}
% \includegraphics[width=.6\linewidth]{imgs/mobilenetv2_8bit_fraclens.pdf}
% \caption{
% \todo{Formats vs layer}
% }
% \label{fig:format_vs_layer}
% \vskip -3ex
% \end{figure*}




==> figs/fig_std_of_model.tex <==
\begin{figure*}[t]
\centering
% \vspace*{-8ex}
% \hspace*{1ex}
\begin{subfigure}[t]{.49\linewidth}
\centering
\includegraphics[width=.8\linewidth]{imgs/placeholder.png}
\caption{\todo{std weight}.}
\label{fig:std_weight}
\end{subfigure}
\hskip 0.4ex
\begin{subfigure}[t]{.49\linewidth}
\centering
\includegraphics[width=.8\linewidth]{imgs/placeholder.png}
\caption{\todo{std act}.}
\label{fig:std_act}
\end{subfigure}
\caption{
\todo{Standard deviation of weight and activation for }
}
\label{fig:std_model}
\vskip -3ex
\end{figure*}

==> tabs/tab_mbv1_conventional.tex <==
\begin{table}[t]
\caption{Comparison on conventional training method.}
\label{tab:liter_comp_both_quant_mbnet}
\begin{center}
\scalebox{.8}{
\begin{tabular}{lccccc}
\toprule
\multicolumn{2}{c}{}&\multicolumn{2}{c}{MobileNet-V1}&\multicolumn{2}{c}{MobileNet-V2}
\\ \cmidrule(r){3-4} \cmidrule(l){5-6}
\multicolumn{1}{c}{Quant. Method} & Bit-widths & Acc.-1 & Acc.-5 & Acc.-1 & Acc.-5
\\ \midrule
PACT & 4bits & 70.3 & 89.2 & 70.4 & 89.4
\\
HAQ & flexible & 67.40 & 87.90 & 66.99 & 87.33
\\
SAT (Ours) & 4bits & {\bf 71.3} & {\bf 89.9} & {\bf 71.1} & {\bf 90.0}
\\ \midrule
PACT & 5bits & 71.1 & 89.6 & 71.2 & 89.8
\\
HAQ & flexible & 70.58 & 89.77 & 70.90 & 89.91
\\
SAT (Ours) & 5bits & {\bf 71.9} & {\bf 90.3} & {\bf 72.0} & {\bf 90.4}
\\ \midrule
PACT & 6bits & 71.2 & 89.2 & 71.5 & 90.0
\\
HAQ & flexible & 71.20 & 90.19 & 71.89 & 90.36
\\
SAT (Ours) & 6bits & {\bf 72.3} & {\bf 90.4} & {\bf 72.3} & {\bf 90.6}
\\ \midrule
PACT & 8bits & 71.3 & 89.7 & 71.7 & 89.9
\\
HAQ & flexible & 70.82 & 89.85 & 71.81 & 90.25
\\
SAT (Ours) & 8bits & {\bf 72.6} & {\bf 90.7} & {\bf 72.5} & {\bf 90.7}
\\ \midrule
PACT & FP & 72.1 & 90.2 & 72.1 & 90.5
\\
SAT (Ours) & FP & 71.7 & 90.2 & 71.8 & 90.2
\\
\bottomrule
\end{tabular}}
\end{center}
\end{table}

==> tabs/tab_res18_conventional.tex <==
\begin{table}[t]
\caption{8-bit ResNet18.}
\label{tab:res18_conventional}
\begin{center}
\scalebox{.8}{
\begin{tabular}{lccccc}
\toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Int} & 8-bit & \multirow{2}{*}{BL} & \multirow{2}{*}{Top-1}
Method & Int & 8-bit & BL & Top-1
% \\
% & & Mult. Only & & &
\\\midrule
\rowcolor{hlrowcolor}
Baseline & \redxmark & \redxmark & 70.3 & 70.3
\\

\bottomrule
\end{tabular}}
\end{center}
\end{table}

==> tex_files/acknowledgement.tex <==
\section{Acknowledgement}
%The Authors would like to appreciate . Also t
This research is partially supported by.

==> tex_files/bak_analysis_PACT_fixed_point.tex <==


% ======================= V3 ========================

\begin{subequations}
\allowdisplaybreaks
\begin{alignat}{3}
    \text{Nonlinear:}\quad&\widetilde{x}^{(l)}_i &&= \clip{\left(x^{(l-1)}_i,0,\alpha^{(l)}\right)}\\
    \text{Input Quant (uint8):}\quad&q^{(l)}_i&&=q\left(\frac{M^{(l)}}{\alpha^{(l)}}\widetilde{x}^{(l)}_i,B_x^{(l)}\right)\\
    \text{Input Dequant:}\quad&\widetilde{q}^{(l)}_i &&=\frac{\alpha^{(l)}}{M^{(l)}}q^{(l)}_i\\
    \text{Conv:}\quad&y^{(l)}_i &&=\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}\widetilde{q}^{(l)}_j\\
    \text{BN:}\quad&x^{(l)}_i&&= \gamma^{(l)}_i\frac{y^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i} + \beta^{(l)}_i\\
    &&&=\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}y^{(l)}_i+
    \left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)
    % z^{(l)}_i &=\eta^{(l)}\widetilde{z}^{(l)}_i\\
    % \widetilde{z}^{(l)}_i &=\rho^{(l)}\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\\
    % \mathrm{d}\widetilde{z}^{(l)}_i &=\xi^{(l)}\cdot\mathrm{d}\left(\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\right)
\end{alignat}
\end{subequations}



\begin{equation}
    \widehat{q}^{(l+1)}_i=\widehat{q}\left(\clip{\left(\sum_{j=1}^{n^{(l)}}\textcolor{\weightcolor}{\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\frac{\alpha^{(l)}}{\lambda^{(l)}}W^{(l)}_{ij}}\textcolor{\inputcolor}{\widehat{q}^{(l)}_j}+
    \textcolor{\biascolor}{\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)},0,\lambda^{(l+1)}\right)},B_x^{(l+1)}\right)
\end{equation}

% ======================= End of V3 ========================


% ======================= V2 ========================

% \begin{subequations}
% \allowdisplaybreaks
% \begin{alignat}{3}
%     \text{Nonlinear:}\quad&\widetilde{x}^{(l)}_i &&= \clip{\left(x^{(l-1)}_i,0,\alpha^{(l)}\right)}\\
%     \text{Input Quant (uint8):}\quad&q^{(l)}_i&&=q\left(\frac{M^{(l)}}{\alpha^{(l)}}\widetilde{x}^{(l)}_i,B_x^{(l)}\right)\\
%     \text{Input Dequant:}\quad&\widetilde{q}^{(l)}_i &&=\frac{\alpha^{(l)}}{M^{(l)}}q^{(l)}_i\\
%     \text{Weight Quant (int8):}\quad&Q^{(l)}_{ij}&&=q\left(\frac{N^{(l)}}{s^{(l)}}\widetilde{W}^{(l)}_{ij},B_w^{(l)}\right)\\
%     \text{Weight Dequant:}\quad&\widetilde{Q}^{(l)}_{ij}&&=\frac{s^{(l)}}{N^{(l)}}Q^{(l)}_{ij}\\
%     \text{Conv:}\quad&y^{(l)}_i &&=\sum_{j=1}^{n^{(l)}}\widetilde{Q}^{(l)}_{ij}\widetilde{q}^{(l)}_j\\
%     \text{BN:}\quad&x^{(l)}_i&&= \gamma^{(l)}_i\frac{y^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i} + \beta^{(l)}_i\\
%     &&&=\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}y^{(l)}_i+
%     \left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)
%     % z^{(l)}_i &=\eta^{(l)}\widetilde{z}^{(l)}_i\\
%     % \widetilde{z}^{(l)}_i &=\rho^{(l)}\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\\
%     % \mathrm{d}\widetilde{z}^{(l)}_i &=\xi^{(l)}\cdot\mathrm{d}\left(\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\right)
% \end{alignat}
% \end{subequations}



% \begin{equation}
%     \widehat{q}^{(l+1)}_i=\widehat{q}\left(\clip{\left(\sum_{j=1}^{n^{(l)}}\textcolor{red}{\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\frac{\alpha^{(l)}}{\lambda^{(l)}}\widetilde{Q}^{(l)}_{ij}}\textcolor{blue}{\widehat{q}^{(l)}_j}+
%     \textcolor{purple}{\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)},0,\lambda^{(l+1)}\right)},B_x^{(l+1)}\right)
% \end{equation}

% ======================= End of V2 ========================


% ======================= V1 ========================

% \begin{subequations}
% \allowdisplaybreaks
% \begin{alignat}{3}
%     \text{Nonlinear:}\quad&\widetilde{x}^{(l)}_i &&= \clip{\left(x^{(l-1)}_i,0,\alpha^{(l)}\right)}\\
%     \text{Input Quant (uint8):}\quad&q^{(l)}_i&&=q\left(\frac{M^{(l)}}{\alpha^{(l)}}\widetilde{x}^{(l)}_i,B_x^{(l)}\right)\\
%     \text{Input Dequant:}\quad&\widetilde{q}^{(l)}_i &&=\frac{\alpha^{(l)}}{M^{(l)}}q^{(l)}_i\\
%     \text{Weight Quant (int8):}\quad&Q^{(l)}_{ij}&&=q\left(\frac{N^{(l)}}{s^{(l)}}\widetilde{W}^{(l)}_{ij},B_w^{(l)}\right)\\
%     \text{Weight Dequant:}\quad&\widetilde{Q}^{(l)}_{ij}&&=\frac{s^{(l)}}{N^{(l)}}Q^{(l)}_{ij}\\
%     \text{Conv:}\quad&y^{(l)}_i &&=\sum_{j=1}^{n^{(l)}}\widetilde{Q}^{(l)}_{ij}\widetilde{q}^{(l)}_j\\
%     \text{BN:}\quad&x^{(l)}_i&&= \gamma^{(l)}_i\frac{y^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i} + \beta^{(l)}_i\\
%     &&&=\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}y^{(l)}_i+
%     \left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)
%     % z^{(l)}_i &=\eta^{(l)}\widetilde{z}^{(l)}_i\\
%     % \widetilde{z}^{(l)}_i &=\rho^{(l)}\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\\
%     % \mathrm{d}\widetilde{z}^{(l)}_i &=\xi^{(l)}\cdot\mathrm{d}\left(\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\right)
% \end{alignat}
% \end{subequations}



% \begin{equation}
%     \widehat{q}^{(l+1)}_i=\widehat{q}\left(\clip{\left(\sum_{j=1}^{n^{(l)}}\textcolor{red}{\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\frac{s^{(l)}}{N^{(l)}}\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\frac{\alpha^{(l)}}{\lambda^{(l)}}Q^{(l)}_{ij}}\textcolor{blue}{\widehat{q}^{(l)}_j}+
%     \textcolor{purple}{\frac{\lambda^{(l+1)}}{\alpha^{(l+1)}}\left(\beta^{(l)}_i-\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\mu^{(l)}_i\right)},0,\lambda^{(l+1)}\right)},B_x^{(l+1)}\right)
% \end{equation}

% ======================= End of V1 ========================


\begin{equation}
    \mathrm{fix\_quant}(x)=\frac{1}{2^\mathrm{fl}}\round\left(\clip\left(x \cdot 2^\mathrm{fl}, 0, 2^\mathrm{wl} - 1\right)\right)
\end{equation}

\begin{equation}
    \mathrm{PACT}(x) = \frac{\alpha}{M}\round\left(\frac{M}{\alpha}\clip\left(x, 0, \alpha\right)\right)
\end{equation}

\begin{equation}
    \mathrm{PACT}(x) = 
    \frac{2^\mathrm{wl}-1}{M}\frac{2^\mathrm{fl}\alpha}{2^\mathrm{wl}-1}\frac{1}{2^\mathrm{fl}}\round\left(\frac{M}{2^\mathrm{wl}-1}\clip\left(\frac{2^\mathrm{wl} - 1}{2^\mathrm{fl}\alpha}x \cdot 2^\mathrm{fl}, 0, 2^\mathrm{wl} - 1\right)\right)
\end{equation}

If $M=2^\mathrm{wl}-1$, we have
\begin{equation}
    \mathrm{PACT}(x) = \frac{2^\mathrm{fl}\alpha}{2^\mathrm{wl}-1}\mathrm{fix\_quant}(\frac{2^\mathrm{wl}-1}{2^\mathrm{fl}\alpha}x)
\end{equation}



